Implications of Clinical Target Distribution Weighted Radiotherapy Optimization

Delineating and planning with respect to regions suspected to contain microscopic tumor cells is an inherently uncertain task in radiotherapy. The recently proposed \textit{clinical target distribution} (CTD) is an alternative to the conventional \textit{clinical target volume} (CTV), with initial promise. Previously, using the CTD in planning has primarily been evaluated in comparison to a conventionally defined CTV. We propose to compare the CTD approach against CTV margins of various sizes, dependent on the threshold at which the tumor infiltration probability is considered relevant. First, a theoretical framework is presented, concerned with optimizing the trade-off between the probability of sufficient target coverage and the penalties associated with high dose. From this framework we derive conventional CTV-based planning and contrast it with the CTD approach. The approaches are contextualized further by comparison with established methods for managing geometric uncertainties. Second, for both a one- and a three-dimensional phantom, we compare a set of CTD plans created by varying the target objective function weight against a set of plans created by varying both the target weight and the CTV margin size. The results show that CTD-based planning gives slightly inefficient trade-offs between the evaluation criteria for a case in which near-minimum target dose is the highest priority. However, in a case when sparing a proximal organ at risk is critical, the CTD is better at maintaining sufficiently high dose toward the center of the target. We conclude that CTD-based planning is a computationally efficient method for planning with respect to delineation uncertainties, but that the inevitable effects on the dose distribution should not be disregarded.

==> old_stuff.tex <==
\begin{comment}
The other is the \textit{tumor control probability}

\begin{equation}
    TCP(d(x)) = \prod_{i \in \mathcal{T}} TCP_i(d_i(x)),
    \label{tcp}
\end{equation}

with the voxel-wise $\text{TCP}_i$ given by the model from \cite{webb_model_1993},

\begin{equation}
    TCP_i(d_i(x)) = e^{-n e^{- \alpha d_i(x)}},
\end{equation}

with the parameters $n_i, \alpha$ being the number of tumor cells in the voxel, and the radiation sensitivity, respectively.
\end{comment}
